Language models represent more about emphasis than they can tell you

Prosodic prominence can largely be predicted from text, but part of it depends on how the speaker reads the sentence. We examine how much information about emphasis language models recover from text, whether they can report it when asked, and what the speech signal adds. Using English speech data with automatically derived word-level emphasis labels, we compare frozen and fine-tuned text models, prompted large language models (LLMs) and speech models on the same words. The text models end within about one point of each other, at best 68.8% on the 3-way task, and make many of the same errors. With the prompts we tested, the LLMs do no better than a word-majority baseline, even with 500 examples. While LLM responses contain some contextual information, they contain less than linear probes find in the model representations, and the gap does not close when the answers are recalibrated or the question is asked differently. The best speech model reaches 84.7%. We argue that text determines only part of the emphasis, and that the rest has to be heard. LLMs encode what the text determines, but prompting reveals only part of it: LLMs represent more about where the emphasis falls than they tell us.

==> results/numbers.tex <==
\makeatletter
\providecommand{\resval}[1]{\ifcsname res@#1\endcsname\csname res@#1\endcsname\else\textbf{??}\fi}
\expandafter\def\csname res@agr-gold-prompted\endcsname{59.9}
\expandafter\def\csname res@agr-gold-speech\endcsname{82.7}
\expandafter\def\csname res@agr-gold-text\endcsname{67.9}
\expandafter\def\csname res@agr-prompted-prompted\endcsname{78.3}
\expandafter\def\csname res@agr-speech-speech\endcsname{84.9}
\expandafter\def\csname res@agr-text-prompted\endcsname{68.8}
\expandafter\def\csname res@agr-text-speech\endcsname{70.6}
\expandafter\def\csname res@agr-text-text\endcsname{84.4}
\expandafter\def\csname res@agreement-2\endcsname{77.0}
\expandafter\def\csname res@agreement-3\endcsname{63.8}
\expandafter\def\csname res@agreement-groups\endcsname{390}
\expandafter\def\csname res@agreement-pairs\endcsname{6{,}277}
\expandafter\def\csname res@ap-audio-2\endcsname{51.0}
\expandafter\def\csname res@ap-audio-3\endcsname{39.2}
\expandafter\def\csname res@ap-text-2\endcsname{51.6}
\expandafter\def\csname res@ap-text-3\endcsname{43.1}
\expandafter\def\csname res@azure-cost\endcsname{73.00}
\expandafter\def\csname res@bd-2---audio\endcsname{92.0}
\expandafter\def\csname res@bd-2---diff\endcsname{8.9}
\expandafter\def\csname res@bd-2---text\endcsname{83.1}
\expandafter\def\csname res@bd-2-content-audio\endcsname{90.0}
\expandafter\def\csname res@bd-2-content-diff\endcsname{7.0}
\expandafter\def\csname res@bd-2-content-text\endcsname{83.0}
\expandafter\def\csname res@bd-2-final-audio\endcsname{86.3}
\expandafter\def\csname res@bd-2-final-diff\endcsname{8.0}
\expandafter\def\csname res@bd-2-final-text\endcsname{78.3}
\expandafter\def\csname res@bd-2-function-audio\endcsname{92.0}
\expandafter\def\csname res@bd-2-function-diff\endcsname{8.9}
\expandafter\def\csname res@bd-2-function-text\endcsname{83.1}
\expandafter\def\csname res@bd-2-given-audio\endcsname{88.5}
\expandafter\def\csname res@bd-2-given-diff\endcsname{9.3}
\expandafter\def\csname res@bd-2-given-text\endcsname{79.3}
\expandafter\def\csname res@bd-2-initial-audio\endcsname{89.2}
\expandafter\def\csname res@bd-2-initial-diff\endcsname{11.0}
\expandafter\def\csname res@bd-2-initial-text\endcsname{78.2}
\expandafter\def\csname res@bd-2-medial-audio\endcsname{91.5}
\expandafter\def\csname res@bd-2-medial-diff\endcsname{7.8}
\expandafter\def\csname res@bd-2-medial-text\endcsname{83.7}
\expandafter\def\csname res@bd-2-new-audio\endcsname{90.6}
\expandafter\def\csname res@bd-2-new-diff\endcsname{6.0}
\expandafter\def\csname res@bd-2-new-text\endcsname{84.6}
\expandafter\def\csname res@bd-3---audio\endcsname{89.5}
\expandafter\def\csname res@bd-3---diff\endcsname{10.8}
\expandafter\def\csname res@bd-3---text\endcsname{78.7}
\expandafter\def\csname res@bd-3-all-right-audio\endcsname{97.1}
\expandafter\def\csname res@bd-3-all-right-diff\endcsname{-2.9}
\expandafter\def\csname res@bd-3-all-right-text\endcsname{100.0}
\expandafter\def\csname res@bd-3-all-wrong-audio\endcsname{58.9}
\expandafter\def\csname res@bd-3-all-wrong-diff\endcsname{58.9}
\expandafter\def\csname res@bd-3-all-wrong-text\endcsname{0.0}
\expandafter\def\csname res@bd-3-content-audio\endcsname{79.0}
\expandafter\def\csname res@bd-3-content-diff\endcsname{22.9}
\expandafter\def\csname res@bd-3-content-text\endcsname{56.1}
\expandafter\def\csname res@bd-3-final-audio\endcsname{75.1}
\expandafter\def\csname res@bd-3-final-diff\endcsname{23.4}
\expandafter\def\csname res@bd-3-final-text\endcsname{51.7}
\expandafter\def\csname res@bd-3-function-audio\endcsname{89.5}
\expandafter\def\csname res@bd-3-function-diff\endcsname{10.8}
\expandafter\def\csname res@bd-3-function-text\endcsname{78.7}
\expandafter\def\csname res@bd-3-given-audio\endcsname{78.8}
\expandafter\def\csname res@bd-3-given-diff\endcsname{23.5}
\expandafter\def\csname res@bd-3-given-text\endcsname{55.3}
\expandafter\def\csname res@bd-3-initial-audio\endcsname{83.4}
\expandafter\def\csname res@bd-3-initial-diff\endcsname{16.4}
\expandafter\def\csname res@bd-3-initial-text\endcsname{67.0}
\expandafter\def\csname res@bd-3-medial-audio\endcsname{85.2}
\expandafter\def\csname res@bd-3-medial-diff\endcsname{16.1}
\expandafter\def\csname res@bd-3-medial-text\endcsname{69.1}
\expandafter\def\csname res@bd-3-new-audio\endcsname{79.1}
\expandafter\def\csname res@bd-3-new-diff\endcsname{22.7}
\expandafter\def\csname res@bd-3-new-text\endcsname{56.4}
\expandafter\def\csname res@bd-3-split-audio\endcsname{80.2}
\expandafter\def\csname res@bd-3-split-diff\endcsname{22.8}
\expandafter\def\csname res@bd-3-split-text\endcsname{57.4}
\expandafter\def\csname res@bertprobe-2\endcsname{81.8}
\expandafter\def\csname res@bertprobe-3\endcsname{64.6}
\expandafter\def\csname res@bilstm-audio-2\endcsname{91.0}
\expandafter\def\csname res@bilstm-audio-3\endcsname{84.7}
\expandafter\def\csname res@bilstm-audio-model-2\endcsname{Whisper large-v3 (encoder)}
\expandafter\def\csname res@bilstm-audio-model-3\endcsname{Whisper large-v3 (encoder)}
\expandafter\def\csname res@bilstm-text-2\endcsname{83.0}
\expandafter\def\csname res@bilstm-text-3\endcsname{68.0}
\expandafter\def\csname res@bilstm-text-model-2\endcsname{ModernBERT-large}
\expandafter\def\csname res@bilstm-text-model-3\endcsname{Qwen3.5 0.8B, echo}
\expandafter\def\csname res@bound-high-2\endcsname{87.7}
\expandafter\def\csname res@bound-high-2-cihi\endcsname{88.4}
\expandafter\def\csname res@bound-high-2-cilo\endcsname{87.0}
\expandafter\def\csname res@bound-high-3\endcsname{79.9}
\expandafter\def\csname res@bound-high-3-cihi\endcsname{80.7}
\expandafter\def\csname res@bound-high-3-cilo\endcsname{79.0}
\expandafter\def\csname res@bound-low-2\endcsname{77.0}
\expandafter\def\csname res@bound-low-2-cihi\endcsname{78.1}
\expandafter\def\csname res@bound-low-2-cilo\endcsname{75.8}
\expandafter\def\csname res@bound-low-3\endcsname{63.8}
\expandafter\def\csname res@bound-low-3-cihi\endcsname{65.1}
\expandafter\def\csname res@bound-low-3-cilo\endcsname{62.4}
\expandafter\def\csname res@bound-texts\endcsname{390}
\expandafter\def\csname res@ceiling-2\endcsname{82.3}
\expandafter\def\csname res@ceiling-3\endcsname{75.0}
\expandafter\def\csname res@ceiling-groups\endcsname{5}
\expandafter\def\csname res@ceiling-readings\endcsname{20}
\expandafter\def\csname res@ceiling-test-utterances\endcsname{0}
\expandafter\def\csname res@ceiling-words\endcsname{124}
\expandafter\def\csname res@cls-deepseek-conf-00\endcsname{80.0}
\expandafter\def\csname res@cls-deepseek-conf-01\endcsname{10.0}
\expandafter\def\csname res@cls-deepseek-conf-02\endcsname{9.9}
\expandafter\def\csname res@cls-deepseek-conf-10\endcsname{28.9}
\expandafter\def\csname res@cls-deepseek-conf-11\endcsname{31.1}
\expandafter\def\csname res@cls-deepseek-conf-12\endcsname{40.0}
\expandafter\def\csname res@cls-deepseek-conf-20\endcsname{13.5}
\expandafter\def\csname res@cls-deepseek-conf-21\endcsname{31.5}
\expandafter\def\csname res@cls-deepseek-conf-22\endcsname{55.1}
\expandafter\def\csname res@cls-deepseek-f1\endcsname{54.7}
\expandafter\def\csname res@cls-deepseek-recall-0\endcsname{80.0}
\expandafter\def\csname res@cls-deepseek-recall-1\endcsname{31.1}
\expandafter\def\csname res@cls-deepseek-recall-2\endcsname{55.1}
\expandafter\def\csname res@cls-gpt4o-conf-00\endcsname{75.4}
\expandafter\def\csname res@cls-gpt4o-conf-01\endcsname{14.6}
\expandafter\def\csname res@cls-gpt4o-conf-02\endcsname{10.0}
\expandafter\def\csname res@cls-gpt4o-conf-10\endcsname{22.5}
\expandafter\def\csname res@cls-gpt4o-conf-11\endcsname{36.7}
\expandafter\def\csname res@cls-gpt4o-conf-12\endcsname{40.8}
\expandafter\def\csname res@cls-gpt4o-conf-20\endcsname{9.6}
\expandafter\def\csname res@cls-gpt4o-conf-21\endcsname{36.9}
\expandafter\def\csname res@cls-gpt4o-conf-22\endcsname{53.5}
\expandafter\def\csname res@cls-gpt4o-f1\endcsname{54.9}
\expandafter\def\csname res@cls-gpt4o-recall-0\endcsname{75.4}
\expandafter\def\csname res@cls-gpt4o-recall-1\endcsname{36.7}
\expandafter\def\csname res@cls-gpt4o-recall-2\endcsname{53.5}
\expandafter\def\csname res@cls-modernbert-conf-00\endcsname{83.5}
\expandafter\def\csname res@cls-modernbert-conf-01\endcsname{11.8}
\expandafter\def\csname res@cls-modernbert-conf-02\endcsname{4.7}
\expandafter\def\csname res@cls-modernbert-conf-10\endcsname{26.6}
\expandafter\def\csname res@cls-modernbert-conf-11\endcsname{45.2}
\expandafter\def\csname res@cls-modernbert-conf-12\endcsname{28.1}
\expandafter\def\csname res@cls-modernbert-conf-20\endcsname{9.0}
\expandafter\def\csname res@cls-modernbert-conf-21\endcsname{27.8}
\expandafter\def\csname res@cls-modernbert-conf-22\endcsname{63.1}
\expandafter\def\csname res@cls-modernbert-f1\endcsname{63.9}
\expandafter\def\csname res@cls-modernbert-recall-0\endcsname{83.5}
\expandafter\def\csname res@cls-modernbert-recall-1\endcsname{45.2}
\expandafter\def\csname res@cls-modernbert-recall-2\endcsname{63.1}
\expandafter\def\csname res@cls-qwen-conf-00\endcsname{83.2}
\expandafter\def\csname res@cls-qwen-conf-01\endcsname{12.6}
\expandafter\def\csname res@cls-qwen-conf-02\endcsname{4.2}
\expandafter\def\csname res@cls-qwen-conf-10\endcsname{26.5}
\expandafter\def\csname res@cls-qwen-conf-11\endcsname{48.4}
\expandafter\def\csname res@cls-qwen-conf-12\endcsname{25.0}
\expandafter\def\csname res@cls-qwen-conf-20\endcsname{9.1}
\expandafter\def\csname res@cls-qwen-conf-21\endcsname{31.7}
\expandafter\def\csname res@cls-qwen-conf-22\endcsname{59.2}
\expandafter\def\csname res@cls-qwen-f1\endcsname{63.8}
\expandafter\def\csname res@cls-qwen-icl-conf-00\endcsname{84.2}
\expandafter\def\csname res@cls-qwen-icl-conf-01\endcsname{10.0}
\expandafter\def\csname res@cls-qwen-icl-conf-02\endcsname{5.8}
\expandafter\def\csname res@cls-qwen-icl-conf-10\endcsname{35.8}
\expandafter\def\csname res@cls-qwen-icl-conf-11\endcsname{35.4}
\expandafter\def\csname res@cls-qwen-icl-conf-12\endcsname{28.8}
\expandafter\def\csname res@cls-qwen-icl-conf-20\endcsname{17.6}
\expandafter\def\csname res@cls-qwen-icl-conf-21\endcsname{34.1}
\expandafter\def\csname res@cls-qwen-icl-conf-22\endcsname{48.3}
\expandafter\def\csname res@cls-qwen-icl-f1\endcsname{55.9}
\expandafter\def\csname res@cls-qwen-icl-recall-0\endcsname{84.2}
\expandafter\def\csname res@cls-qwen-icl-recall-1\endcsname{35.4}
\expandafter\def\csname res@cls-qwen-icl-recall-2\endcsname{48.3}
\expandafter\def\csname res@cls-qwen-recall-0\endcsname{83.2}
\expandafter\def\csname res@cls-qwen-recall-1\endcsname{48.4}
\expandafter\def\csname res@cls-qwen-recall-2\endcsname{59.2}
\expandafter\def\csname res@cls-whisper-conf-00\endcsname{90.4}
\expandafter\def\csname res@cls-whisper-conf-01\endcsname{9.1}
\expandafter\def\csname res@cls-whisper-conf-02\endcsname{0.6}
\expandafter\def\csname res@cls-whisper-conf-10\endcsname{14.1}
\expandafter\def\csname res@cls-whisper-conf-11\endcsname{72.4}
\expandafter\def\csname res@cls-whisper-conf-12\endcsname{13.5}
\expandafter\def\csname res@cls-whisper-conf-20\endcsname{1.3}
\expandafter\def\csname res@cls-whisper-conf-21\endcsname{12.2}
\expandafter\def\csname res@cls-whisper-conf-22\endcsname{86.6}
\expandafter\def\csname res@cls-whisper-f1\endcsname{83.0}
\expandafter\def\csname res@cls-whisper-recall-0\endcsname{90.4}
\expandafter\def\csname res@cls-whisper-recall-1\endcsname{72.4}
\expandafter\def\csname res@cls-whisper-recall-2\endcsname{86.6}
\expandafter\def\csname res@common-audio-2\endcsname{90.9}
\expandafter\def\csname res@common-audio-3\endcsname{84.6}
\expandafter\def\csname res@common-audio-system-2\endcsname{whisper-large-v3 (audio-mean) bilstm}
\expandafter\def\csname res@common-audio-system-3\endcsname{whisper-large-v3 (audio-mean) bilstm}
\expandafter\def\csname res@common-share\endcsname{99.9}
\expandafter\def\csname res@common-text-2\endcsname{83.1}
\expandafter\def\csname res@common-text-3\endcsname{68.1}
\expandafter\def\csname res@common-text-system-2\endcsname{modernbert-large (plain-first-natural) bilstm}
\expandafter\def\csname res@common-text-system-3\endcsname{qwen3.5-0.8b-base (echo-last-natural) bilstm}
\expandafter\def\csname res@common-words\endcsname{89{,}935}
\expandafter\def\csname res@consensus-acc-2\endcsname{82.0}
\expandafter\def\csname res@consensus-acc-3\endcsname{66.5}
\expandafter\def\csname res@consensus-mutual-2\endcsname{94.0}
\expandafter\def\csname res@consensus-mutual-3\endcsname{82.6}
\expandafter\def\csname res@consensus-shared-errors-2\endcsname{45.2}
\expandafter\def\csname res@consensus-shared-errors-3\endcsname{18.7}
\expandafter\def\csname res@consensus-systems\endcsname{42}
\expandafter\def\csname res@consensus-unanimous-2\endcsname{74.4}
\expandafter\def\csname res@consensus-unanimous-3\endcsname{45.8}
\expandafter\def\csname res@consensus-unanimous-wrong-2\endcsname{8.1}
\expandafter\def\csname res@consensus-unanimous-wrong-3\endcsname{6.3}
\expandafter\def\csname res@corpus-negative\endcsname{0}
\expandafter\def\csname res@corpus-words\endcsname{2{,}265{,}552}
\expandafter\def\csname res@corpus-zero-share\endcsname{9.3}
\expandafter\def\csname res@ctl-layer0-bilstm-2\endcsname{82.5}
\expandafter\def\csname res@ctl-layer0-bilstm-3\endcsname{67.1}
\expandafter\def\csname res@ctl-matched-bilstm-2\endcsname{80.3}
\expandafter\def\csname res@ctl-matched-bilstm-3\endcsname{63.2}
\expandafter\def\csname res@ctl-matched-lin-2\endcsname{80.7}
\expandafter\def\csname res@ctl-matched-lin-3\endcsname{63.0}
\expandafter\def\csname res@ctl-qwen-layer0-bilstm-2\endcsname{82.3}
\expandafter\def\csname res@ctl-qwen-layer0-bilstm-3\endcsname{66.5}
\expandafter\def\csname res@ctl-random-bilstm-2\endcsname{82.5}
\expandafter\def\csname res@ctl-random-bilstm-3\endcsname{66.6}
\expandafter\def\csname res@ctx-bert-plain-bilstm-2\endcsname{82.9}
\expandafter\def\csname res@ctx-bert-plain-bilstm-3\endcsname{67.7}
\expandafter\def\csname res@ctx-bert-plain-lin-2\endcsname{81.8}
\expandafter\def\csname res@ctx-bert-plain-lin-3\endcsname{64.6}
\expandafter\def\csname res@ctx-bert-prev1-bilstm-2\endcsname{83.0}
\expandafter\def\csname res@ctx-bert-prev1-bilstm-3\endcsname{67.7}
\expandafter\def\csname res@ctx-bert-prev1-bilstm-gain-2\endcsname{0.0}
\expandafter\def\csname res@ctx-bert-prev1-bilstm-gain-3\endcsname{0.0}
\expandafter\def\csname res@ctx-bert-prev1-lin-2\endcsname{81.7}
\expandafter\def\csname res@ctx-bert-prev1-lin-3\endcsname{64.7}
\expandafter\def\csname res@ctx-bert-prev1-lin-gain-2\endcsname{-0.1}
\expandafter\def\csname res@ctx-bert-prev1-lin-gain-3\endcsname{0.1}
\expandafter\def\csname res@ctx-bert-prev3-bilstm-2\endcsname{82.9}
\expandafter\def\csname res@ctx-bert-prev3-bilstm-3\endcsname{67.7}
\expandafter\def\csname res@ctx-bert-prev3-bilstm-gain-2\endcsname{0.0}
\expandafter\def\csname res@ctx-bert-prev3-bilstm-gain-3\endcsname{0.0}
\expandafter\def\csname res@ctx-bert-prev3-lin-2\endcsname{81.8}
\expandafter\def\csname res@ctx-bert-prev3-lin-3\endcsname{64.7}
\expandafter\def\csname res@ctx-bert-prev3-lin-gain-2\endcsname{0.0}
\expandafter\def\csname res@ctx-bert-prev3-lin-gain-3\endcsname{0.1}
\expandafter\def\csname res@ctx-max-gain-3\endcsname{0.1}
\expandafter\def\csname res@ctx-modernbert-plain-bilstm-2\endcsname{83.0}
\expandafter\def\csname res@ctx-modernbert-plain-bilstm-3\endcsname{68.0}
\expandafter\def\csname res@ctx-modernbert-plain-lin-2\endcsname{81.9}
\expandafter\def\csname res@ctx-modernbert-plain-lin-3\endcsname{65.3}
\expandafter\def\csname res@ctx-modernbert-prev3-bilstm-2\endcsname{83.0}
\expandafter\def\csname res@ctx-modernbert-prev3-bilstm-3\endcsname{67.9}
\expandafter\def\csname res@ctx-modernbert-prev3-bilstm-gain-2\endcsname{-0.1}
\expandafter\def\csname res@ctx-modernbert-prev3-bilstm-gain-3\endcsname{-0.1}
\expandafter\def\csname res@ctx-modernbert-prev3-lin-2\endcsname{81.9}
\expandafter\def\csname res@ctx-modernbert-prev3-lin-3\endcsname{65.3}
\expandafter\def\csname res@ctx-modernbert-prev3-lin-gain-2\endcsname{0.0}
\expandafter\def\csname res@ctx-modernbert-prev3-lin-gain-3\endcsname{0.1}
\expandafter\def\csname res@data-dev-speakers\endcsname{40}
\expandafter\def\csname res@data-dev-utts\endcsname{5{,}727}
\expandafter\def\csname res@data-dev-words\endcsname{99{,}200}
\expandafter\def\csname res@data-shared-speakers\endcsname{0}
\expandafter\def\csname res@data-test-speakers\endcsname{39}
\expandafter\def\csname res@data-test-utts\endcsname{4{,}822}
\expandafter\def\csname res@data-test-words\endcsname{90{,}063}
\expandafter\def\csname res@data-train100-speakers\endcsname{245}
\expandafter\def\csname res@data-train100-utts\endcsname{33{,}042}
\expandafter\def\csname res@data-train100-words\endcsname{570{,}592}
\expandafter\def\csname res@data-train360-speakers\endcsname{904}
\expandafter\def\csname res@data-train360-utts\endcsname{116{,}263}
\expandafter\def\csname res@data-train360-words\endcsname{2{,}076{,}289}
\expandafter\def\csname res@decoders-probed\endcsname{8}
\expandafter\def\csname res@duration-2\endcsname{83.2}
\expandafter\def\csname res@duration-3\endcsname{65.0}
\expandafter\def\csname res@echo-gain-max-2\endcsname{0.4}
\expandafter\def\csname res@echo-gain-max-3\endcsname{1.2}
\expandafter\def\csname res@echo-gain-min-2\endcsname{0.2}
\expandafter\def\csname res@echo-gain-min-3\endcsname{0.8}
\expandafter\def\csname res@emb-bert-2\endcsname{80.8}
\expandafter\def\csname res@emb-bert-3\endcsname{62.4}
\expandafter\def\csname res@emb-qwen-2\endcsname{81.2}
\expandafter\def\csname res@emb-qwen-3\endcsname{62.9}
\expandafter\def\csname res@encoders-probed\endcsname{7}
\expandafter\def\csname res@fg-audio-enumeration\endcsname{14}
\expandafter\def\csname res@fg-audio-labelled\endcsname{94}
\expandafter\def\csname res@fg-audio-labels\endcsname{4}
\expandafter\def\csname res@fg-audio-n\endcsname{20}
\expandafter\def\csname res@fg-audio-other\endcsname{2}
\expandafter\def\csname res@fg-audio-zero\endcsname{93}
\expandafter\def\csname res@fg-text-enumeration\endcsname{9}
\expandafter\def\csname res@fg-text-labelled\endcsname{183}
\expandafter\def\csname res@fg-text-labels\endcsname{10}
\expandafter\def\csname res@fg-text-n\endcsname{20}
\expandafter\def\csname res@fg-text-other\endcsname{1}
\expandafter\def\csname res@fg-text-zero\endcsname{180}
\expandafter\def\csname res@ft-bert-large-uncased-2\endcsname{83.1}
\expandafter\def\csname res@ft-bert-large-uncased-3\endcsname{68.5}
\expandafter\def\csname res@ft-bert-large-uncased-sd-2\endcsname{0.09}
\expandafter\def\csname res@ft-bert-large-uncased-sd-3\endcsname{0.13}
\expandafter\def\csname res@ft-modernbert-large-2\endcsname{83.2}
\expandafter\def\csname res@ft-modernbert-large-3\endcsname{68.8}
\expandafter\def\csname res@ft-modernbert-large-sd-2\endcsname{0.05}
\expandafter\def\csname res@ft-modernbert-large-sd-3\endcsname{0.08}
\expandafter\def\csname res@ft-xlm-roberta-large-2\endcsname{83.3}
\expandafter\def\csname res@ft-xlm-roberta-large-3\endcsname{68.8}
\expandafter\def\csname res@ft-xlm-roberta-large-sd-2\endcsname{0.11}
\expandafter\def\csname res@ft-xlm-roberta-large-sd-3\endcsname{0.17}
\expandafter\def\csname res@gap-2\endcsname{7.8}
\expandafter\def\csname res@gap-3\endcsname{16.5}
\expandafter\def\csname res@gap-best-2\endcsname{7.8}
\expandafter\def\csname res@gap-best-3\endcsname{15.9}
\expandafter\def\csname res@gpu-hours-finetune\endcsname{6.2}
\expandafter\def\csname res@gpu-hours-longest\endcsname{8.1}
\expandafter\def\csname res@gpu-hours-probe\endcsname{34.2}
\expandafter\def\csname res@gpu-hours-prompt\endcsname{18.1}
\expandafter\def\csname res@gpu-hours-total\endcsname{58.5}
\expandafter\def\csname res@gpu-runs\endcsname{106}
\expandafter\def\csname res@icl-dev-0-2\endcsname{79.5}
\expandafter\def\csname res@icl-dev-0-3\endcsname{60.5}
\expandafter\def\csname res@icl-dev-10-2\endcsname{79.3}
\expandafter\def\csname res@icl-dev-10-3\endcsname{61.8}
\expandafter\def\csname res@icl-dev-100-2\endcsname{79.1}
\expandafter\def\csname res@icl-dev-100-3\endcsname{63.1}
\expandafter\def\csname res@icl-dev-25-2\endcsname{79.7}
\expandafter\def\csname res@icl-dev-25-3\endcsname{62.6}
\expandafter\def\csname res@icl-dev-250-2\endcsname{79.0}
\expandafter\def\csname res@icl-dev-250-3\endcsname{63.2}
\expandafter\def\csname res@icl-dev-500-2\endcsname{79.0}
\expandafter\def\csname res@icl-dev-500-3\endcsname{63.5}
\expandafter\def\csname res@icl-probe-f1-gap\endcsname{7.8}
\expandafter\def\csname res@icl-test-2\endcsname{78.3}
\expandafter\def\csname res@icl-test-3\endcsname{62.0}
\expandafter\def\csname res@icl-test-k0-2\endcsname{78.8}
\expandafter\def\csname res@icl-test-k0-3\endcsname{58.6}
\expandafter\def\csname res@lc-bilstm-116263\endcsname{67.7}
\expandafter\def\csname res@lc-bilstm-33042\endcsname{67.1}
\expandafter\def\csname res@lc-finetune-11626\endcsname{66.9}
\expandafter\def\csname res@lc-finetune-116263\endcsname{68.5}
\expandafter\def\csname res@lc-linear-116263\endcsname{64.6}
\expandafter\def\csname res@lc-linear-33042\endcsname{64.4}
\expandafter\def\csname res@lc-linear-500\endcsname{62.7}
\expandafter\def\csname res@lc-linear-5000\endcsname{64.4}
\expandafter\def\csname res@legacy-full-maxdiff\endcsname{0.02}
\expandafter\def\csname res@lex-deepseek-agree\endcsname{68.8}
\expandafter\def\csname res@lex-deepseek-dep_right\endcsname{37.1}
\expandafter\def\csname res@lex-deepseek-dep_wm_right\endcsname{42.1}
\expandafter\def\csname res@lex-deepseek-departs\endcsname{31.2}
\expandafter\def\csname res@lex-gpt4o-agree\endcsname{68.0}
\expandafter\def\csname res@lex-gpt4o-dep_right\endcsname{36.0}
\expandafter\def\csname res@lex-gpt4o-dep_wm_right\endcsname{44.2}
\expandafter\def\csname res@lex-gpt4o-departs\endcsname{32.0}
\expandafter\def\csname res@lex-modernbert-agree\endcsname{71.7}
\expandafter\def\csname res@lex-modernbert-dep_right\endcsname{51.8}
\expandafter\def\csname res@lex-modernbert-dep_wm_right\endcsname{30.7}
\expandafter\def\csname res@lex-modernbert-departs\endcsname{28.3}
\expandafter\def\csname res@lex-qwen-agree\endcsname{72.4}
\expandafter\def\csname res@lex-qwen-dep_right\endcsname{51.4}
\expandafter\def\csname res@lex-qwen-dep_wm_right\endcsname{30.8}
\expandafter\def\csname res@lex-qwen-departs\endcsname{27.6}
\expandafter\def\csname res@lex-qwen-icl-agree\endcsname{69.3}
\expandafter\def\csname res@lex-qwen-icl-dep_right\endcsname{39.5}
\expandafter\def\csname res@lex-qwen-icl-dep_wm_right\endcsname{39.8}
\expandafter\def\csname res@lex-qwen-icl-departs\endcsname{30.7}
\expandafter\def\csname res@lin-audio-2\endcsname{88.2}
\expandafter\def\csname res@lin-audio-3\endcsname{78.7}
\expandafter\def\csname res@lin-audio-model-2\endcsname{Whisper large-v3 (encoder)}
\expandafter\def\csname res@lin-audio-model-3\endcsname{Whisper large-v3 (encoder)}
\expandafter\def\csname res@lin-text-2\endcsname{82.6}
\expandafter\def\csname res@lin-text-3\endcsname{66.9}
\expandafter\def\csname res@lin-text-model-2\endcsname{Muse Glimmer 30B, echo}
\expandafter\def\csname res@lin-text-model-3\endcsname{Muse Glimmer 30B, echo}
\expandafter\def\csname res@majority-2\endcsname{52.0}
\expandafter\def\csname res@majority-3\endcsname{48.0}
\expandafter\def\csname res@mc-0-icl-2\endcsname{79.5}
\expandafter\def\csname res@mc-0-icl-3\endcsname{60.5}
\expandafter\def\csname res@mc-10-icl-2\endcsname{79.3}
\expandafter\def\csname res@mc-10-icl-3\endcsname{61.8}
\expandafter\def\csname res@mc-10-lookup-3\endcsname{45.0}
\expandafter\def\csname res@mc-10-probe-2\endcsname{76.8}
\expandafter\def\csname res@mc-10-probe-3\endcsname{57.4}
\expandafter\def\csname res@mc-100-icl-2\endcsname{79.1}
\expandafter\def\csname res@mc-100-icl-3\endcsname{63.1}
\expandafter\def\csname res@mc-100-lookup-3\endcsname{49.3}
\expandafter\def\csname res@mc-100-probe-2\endcsname{79.5}
\expandafter\def\csname res@mc-100-probe-3\endcsname{61.7}
\expandafter\def\csname res@mc-25-icl-2\endcsname{79.7}
\expandafter\def\csname res@mc-25-icl-3\endcsname{62.6}
\expandafter\def\csname res@mc-25-lookup-3\endcsname{47.1}
\expandafter\def\csname res@mc-25-probe-2\endcsname{78.6}
\expandafter\def\csname res@mc-25-probe-3\endcsname{59.7}
\expandafter\def\csname res@mc-250-icl-2\endcsname{79.0}
\expandafter\def\csname res@mc-250-icl-3\endcsname{63.2}
\expandafter\def\csname res@mc-250-lookup-3\endcsname{50.8}
\expandafter\def\csname res@mc-250-probe-2\endcsname{80.6}
\expandafter\def\csname res@mc-250-probe-3\endcsname{63.4}
\expandafter\def\csname res@mc-500-icl-2\endcsname{79.0}
\expandafter\def\csname res@mc-500-icl-3\endcsname{63.5}
\expandafter\def\csname res@mc-500-lookup-3\endcsname{51.8}
\expandafter\def\csname res@mc-500-probe-2\endcsname{80.7}
\expandafter\def\csname res@mc-500-probe-3\endcsname{63.7}
\expandafter\def\csname res@mc-all-probe-2\endcsname{82.7}
\expandafter\def\csname res@mc-all-probe-3\endcsname{66.8}
\expandafter\def\csname res@overlap-diff-max-2\endcsname{5.8}
\expandafter\def\csname res@overlap-diff-max-3\endcsname{5.5}
\expandafter\def\csname res@overlap-diff-min-2\endcsname{3.2}
\expandafter\def\csname res@overlap-diff-min-3\endcsname{1.6}
\expandafter\def\csname res@overlap-utterances\endcsname{189}
\expandafter\def\csname res@overlap-words\endcsname{2{,}733}
\expandafter\def\csname res@p-bert-bilstm-2\endcsname{82.9}
\expandafter\def\csname res@p-bert-bilstm-3\endcsname{67.7}
\expandafter\def\csname res@p-bert-depth\endcsname{33}
\expandafter\def\csname res@p-bert-layer\endcsname{4/12}
\expandafter\def\csname res@p-bert-lin-2\endcsname{81.8}
\expandafter\def\csname res@p-bert-lin-3\endcsname{64.6}
\expandafter\def\csname res@p-bert100-bilstm-2\endcsname{82.7}
\expandafter\def\csname res@p-bert100-bilstm-3\endcsname{67.1}
\expandafter\def\csname res@p-bert100-depth\endcsname{33}
\expandafter\def\csname res@p-bert100-layer\endcsname{4/12}
\expandafter\def\csname res@p-bert100-lin-2\endcsname{81.8}
\expandafter\def\csname res@p-bert100-lin-3\endcsname{64.4}
\expandafter\def\csname res@p-glimmer-bilstm-2\endcsname{82.8}
\expandafter\def\csname res@p-glimmer-bilstm-3\endcsname{67.9}
\expandafter\def\csname res@p-glimmer-depth\endcsname{19}
\expandafter\def\csname res@p-glimmer-layer\endcsname{10/52}
\expandafter\def\csname res@p-glimmer-lin-2\endcsname{82.6}
\expandafter\def\csname res@p-glimmer-lin-3\endcsname{66.9}
\expandafter\def\csname res@p-glimmer100-bilstm-2\endcsname{82.7}
\expandafter\def\csname res@p-glimmer100-bilstm-3\endcsname{67.5}
\expandafter\def\csname res@p-glimmer100-depth\endcsname{19}
\expandafter\def\csname res@p-glimmer100-layer\endcsname{10/52}
\expandafter\def\csname res@p-glimmer100-lin-2\endcsname{82.5}
\expandafter\def\csname res@p-glimmer100-lin-3\endcsname{66.7}
\expandafter\def\csname res@p-hubert-bilstm-2\endcsname{90.9}
\expandafter\def\csname res@p-hubert-bilstm-3\endcsname{84.1}
\expandafter\def\csname res@p-hubert-depth\endcsname{54}
\expandafter\def\csname res@p-hubert-layer\endcsname{13/24}
\expandafter\def\csname res@p-hubert-lin-2\endcsname{88.2}
\expandafter\def\csname res@p-hubert-lin-3\endcsname{78.8}
\expandafter\def\csname res@p-qaenc-bilstm-2\endcsname{91.0}
\expandafter\def\csname res@p-qaenc-bilstm-3\endcsname{84.2}
\expandafter\def\csname res@p-qaenc-depth\endcsname{69}
\expandafter\def\csname res@p-qaenc-layer\endcsname{22/32}
\expandafter\def\csname res@p-qaenc-lin-2\endcsname{88.1}
\expandafter\def\csname res@p-qaenc-lin-3\endcsname{78.1}
\expandafter\def\csname res@p-qalm-bilstm-2\endcsname{87.3}
\expandafter\def\csname res@p-qalm-bilstm-3\endcsname{76.5}
\expandafter\def\csname res@p-qalm-depth\endcsname{9}
\expandafter\def\csname res@p-qalm-layer\endcsname{3/32}
\expandafter\def\csname res@p-qalm-lin-2\endcsname{86.4}
\expandafter\def\csname res@p-qalm-lin-3\endcsname{74.4}
\expandafter\def\csname res@p-qwen-bilstm-2\endcsname{82.9}
\expandafter\def\csname res@p-qwen-bilstm-3\endcsname{67.8}
\expandafter\def\csname res@p-qwen-depth\endcsname{84}
\expandafter\def\csname res@p-qwen-layer\endcsname{54/64}
\expandafter\def\csname res@p-qwen-lin-2\endcsname{82.3}
\expandafter\def\csname res@p-qwen-lin-3\endcsname{66.7}
\expandafter\def\csname res@p-wavlm-bilstm-2\endcsname{90.6}
\expandafter\def\csname res@p-wavlm-bilstm-3\endcsname{83.9}
\expandafter\def\csname res@p-wavlm-depth\endcsname{54}
\expandafter\def\csname res@p-wavlm-layer\endcsname{13/24}
\expandafter\def\csname res@p-wavlm-lin-2\endcsname{87.8}
\expandafter\def\csname res@p-wavlm-lin-3\endcsname{78.0}
\expandafter\def\csname res@p-whisper-bilstm-2\endcsname{91.0}
\expandafter\def\csname res@p-whisper-bilstm-3\endcsname{84.7}
\expandafter\def\csname res@p-whisper-depth\endcsname{72}
\expandafter\def\csname res@p-whisper-layer\endcsname{23/32}
\expandafter\def\csname res@p-whisper-lin-2\endcsname{88.2}
\expandafter\def\csname res@p-whisper-lin-3\endcsname{78.7}
\expandafter\def\csname res@paper2019-2\endcsname{83.2}
\expandafter\def\csname res@paper2019-3\endcsname{68.6}
\expandafter\def\csname res@pp-deepseek-content-acc\endcsname{44.2}
\expandafter\def\csname res@pp-deepseek-content-gap\endcsname{11.6}
\expandafter\def\csname res@pp-deepseek-content-top\endcsname{56.8}
\expandafter\def\csname res@pp-deepseek-function-acc\endcsname{75.0}
\expandafter\def\csname res@pp-deepseek-function-gap\endcsname{3.4}
\expandafter\def\csname res@pp-deepseek-function-top\endcsname{4.8}
\expandafter\def\csname res@pp-deepseek-last-acc\endcsname{38.3}
\expandafter\def\csname res@pp-deepseek-last-top\endcsname{77.1}
\expandafter\def\csname res@pp-dev-deepseek-linguistic-last-top\endcsname{70.0}
\expandafter\def\csname res@pp-dev-deepseek-minimal-last-top\endcsname{72.6}
\expandafter\def\csname res@pp-dev-deepseek-narrator-last-top\endcsname{53.2}
\expandafter\def\csname res@pp-dev-gold-last-top\endcsname{32.4}
\expandafter\def\csname res@pp-dev-gpt4o-linguistic-last-top\endcsname{71.0}
\expandafter\def\csname res@pp-dev-gpt4o-minimal-last-top\endcsname{73.2}
\expandafter\def\csname res@pp-dev-gpt4o-narrator-last-top\endcsname{70.0}
\expandafter\def\csname res@pp-dev-minimal-last-top-max\endcsname{73.2}
\expandafter\def\csname res@pp-dev-minimal-last-top-min\endcsname{54.4}
\expandafter\def\csname res@pp-dev-mistral-linguistic-last-top\endcsname{48.8}
\expandafter\def\csname res@pp-dev-mistral-minimal-last-top\endcsname{54.4}
\expandafter\def\csname res@pp-dev-mistral-narrator-last-top\endcsname{37.4}
\expandafter\def\csname res@pp-gold-content-acc\endcsname{100.0}
\expandafter\def\csname res@pp-gold-content-top\endcsname{42.2}
\expandafter\def\csname res@pp-gold-function-acc\endcsname{100.0}
\expandafter\def\csname res@pp-gold-function-top\endcsname{9.2}
\expandafter\def\csname res@pp-gold-last-acc\endcsname{100.0}
\expandafter\def\csname res@pp-gold-last-top\endcsname{31.9}
\expandafter\def\csname res@pp-gpt4o-content-acc\endcsname{43.7}
\expandafter\def\csname res@pp-gpt4o-content-gap\endcsname{12.1}
\expandafter\def\csname res@pp-gpt4o-content-top\endcsname{58.7}
\expandafter\def\csname res@pp-gpt4o-function-acc\endcsname{73.5}
\expandafter\def\csname res@pp-gpt4o-function-gap\endcsname{4.9}
\expandafter\def\csname res@pp-gpt4o-function-top\endcsname{2.8}
\expandafter\def\csname res@pp-gpt4o-last-acc\endcsname{37.0}
\expandafter\def\csname res@pp-gpt4o-last-top\endcsname{81.4}
\expandafter\def\csname res@pp-modernbert-content-acc\endcsname{56.1}
\expandafter\def\csname res@pp-modernbert-content-top\endcsname{46.7}
\expandafter\def\csname res@pp-modernbert-function-acc\endcsname{78.7}
\expandafter\def\csname res@pp-modernbert-function-top\endcsname{6.7}
\expandafter\def\csname res@pp-modernbert-last-acc\endcsname{51.7}
\expandafter\def\csname res@pp-modernbert-last-top\endcsname{35.4}
\expandafter\def\csname res@pp-qwen-content-acc\endcsname{55.8}
\expandafter\def\csname res@pp-qwen-content-top\endcsname{43.1}
\expandafter\def\csname res@pp-qwen-function-acc\endcsname{78.4}
\expandafter\def\csname res@pp-qwen-function-top\endcsname{6.0}
\expandafter\def\csname res@pp-qwen-icl-content-acc\endcsname{46.8}
\expandafter\def\csname res@pp-qwen-icl-content-gap\endcsname{9.0}
\expandafter\def\csname res@pp-qwen-icl-content-top\endcsname{44.2}
\expandafter\def\csname res@pp-qwen-icl-function-acc\endcsname{75.6}
\expandafter\def\csname res@pp-qwen-icl-function-gap\endcsname{2.8}
\expandafter\def\csname res@pp-qwen-icl-function-top\endcsname{3.4}
\expandafter\def\csname res@pp-qwen-icl-last-acc\endcsname{43.0}
\expandafter\def\csname res@pp-qwen-icl-last-top\endcsname{45.5}
\expandafter\def\csname res@pp-qwen-last-acc\endcsname{51.3}
\expandafter\def\csname res@pp-qwen-last-top\endcsname{31.7}
\expandafter\def\csname res@pp-whisper-content-acc\endcsname{78.9}
\expandafter\def\csname res@pp-whisper-content-top\endcsname{43.4}
\expandafter\def\csname res@pp-whisper-function-acc\endcsname{89.5}
\expandafter\def\csname res@pp-whisper-function-top\endcsname{9.3}
\expandafter\def\csname res@pp-whisper-last-acc\endcsname{74.9}
\expandafter\def\csname res@pp-whisper-last-top\endcsname{32.7}
\expandafter\def\csname res@profile-probe-gold-0\endcsname{48.0}
\expandafter\def\csname res@profile-probe-gold-1\endcsname{27.3}
\expandafter\def\csname res@profile-probe-gold-2\endcsname{24.7}
\expandafter\def\csname res@profile-probe-pred-0\endcsname{47.1}
\expandafter\def\csname res@profile-probe-pred-1\endcsname{29.1}
\expandafter\def\csname res@profile-probe-pred-2\endcsname{23.9}
\expandafter\def\csname res@profile-probe-recall-0\endcsname{80.6}
\expandafter\def\csname res@profile-probe-recall-1\endcsname{50.2}
\expandafter\def\csname res@profile-probe-recall-2\endcsname{58.7}
\expandafter\def\csname res@profile-prompt-gold-0\endcsname{48.0}
\expandafter\def\csname res@profile-prompt-gold-1\endcsname{27.3}
\expandafter\def\csname res@profile-prompt-gold-2\endcsname{24.7}
\expandafter\def\csname res@profile-prompt-pred-0\endcsname{49.6}
\expandafter\def\csname res@profile-prompt-pred-1\endcsname{21.1}
\expandafter\def\csname res@profile-prompt-pred-2\endcsname{29.3}
\expandafter\def\csname res@profile-prompt-recall-0\endcsname{80.0}
\expandafter\def\csname res@profile-prompt-recall-1\endcsname{31.1}
\expandafter\def\csname res@profile-prompt-recall-2\endcsname{55.1}
\expandafter\def\csname res@prompt-best-2\endcsname{79.7}
\expandafter\def\csname res@prompt-best-3\endcsname{60.5}
\expandafter\def\csname res@prompt-best-model-2\endcsname{GPT-4o}
\expandafter\def\csname res@prompt-best-model-3\endcsname{DeepSeek-V4-Pro}
\expandafter\def\csname res@qa-loss-2\endcsname{3.7}
\expandafter\def\csname res@qa-loss-3\endcsname{7.7}
\expandafter\def\csname res@recon-2\endcsname{95.0}
\expandafter\def\csname res@recon-3\endcsname{91.5}
\expandafter\def\csname res@recon-coverage\endcsname{99.9}
\expandafter\def\csname res@recon-pearson\endcsname{0.978}
\expandafter\def\csname res@recon-spearman\endcsname{0.967}
\expandafter\def\csname res@repro-2\endcsname{83.02}
\expandafter\def\csname res@repro-3\endcsname{68.49}
\expandafter\def\csname res@repro-sd-2\endcsname{0.13}
\expandafter\def\csname res@repro-sd-3\endcsname{0.10}
\expandafter\def\csname res@rt-deepseek-diff\endcsname{0.4}
\expandafter\def\csname res@rt-deepseek-other\endcsname{58.7}
\expandafter\def\csname res@rt-deepseek-own\endcsname{59.1}
\expandafter\def\csname res@rt-dev-k0-argmax\endcsname{60.5}
\expandafter\def\csname res@rt-dev-k0-auc\endcsname{0.856}
\expandafter\def\csname res@rt-dev-k0-cv\endcsname{60.9}
\expandafter\def\csname res@rt-dev-k500-argmax\endcsname{63.5}
\expandafter\def\csname res@rt-dev-k500-auc\endcsname{0.876}
\expandafter\def\csname res@rt-dev-k500-cv\endcsname{63.0}
\expandafter\def\csname res@rt-dev-lex-auc\endcsname{0.874}
\expandafter\def\csname res@rt-dev-wordmaj\endcsname{62.4}
\expandafter\def\csname res@rt-modernbert-diff\endcsname{-3.2}
\expandafter\def\csname res@rt-modernbert-other\endcsname{70.6}
\expandafter\def\csname res@rt-modernbert-own\endcsname{67.4}
\expandafter\def\csname res@rt-qwen-diff\endcsname{-4.2}
\expandafter\def\csname res@rt-qwen-icl-diff\endcsname{-1.2}
\expandafter\def\csname res@rt-qwen-icl-other\endcsname{62.0}
\expandafter\def\csname res@rt-qwen-icl-own\endcsname{60.8}
\expandafter\def\csname res@rt-qwen-other\endcsname{69.9}
\expandafter\def\csname res@rt-qwen-own\endcsname{65.7}
\expandafter\def\csname res@rt-readers\endcsname{64.2}
\expandafter\def\csname res@rt-utterances\endcsname{143}
\expandafter\def\csname res@rt-wavlm-diff\endcsname{15.8}
\expandafter\def\csname res@rt-wavlm-other\endcsname{65.5}
\expandafter\def\csname res@rt-wavlm-own\endcsname{81.3}
\expandafter\def\csname res@rt-whisper-diff\endcsname{14.5}
\expandafter\def\csname res@rt-whisper-other\endcsname{65.8}
\expandafter\def\csname res@rt-whisper-own\endcsname{80.3}
\expandafter\def\csname res@rt-words\endcsname{1{,}906}
\expandafter\def\csname res@sample-between-maxdiff\endcsname{0.0}
\expandafter\def\csname res@sample-own-maxdiff\endcsname{0.2}
\expandafter\def\csname res@sample-own-same\endcsname{15}
\expandafter\def\csname res@sample-public-maxdiff\endcsname{0.2}
\expandafter\def\csname res@sample-public-same\endcsname{15}
\expandafter\def\csname res@sample-words\endcsname{15}
\expandafter\def\csname res@size-0.8-2\endcsname{81.7}
\expandafter\def\csname res@size-0.8-3\endcsname{65.7}
\expandafter\def\csname res@size-2-2\endcsname{82.0}
\expandafter\def\csname res@size-2-3\endcsname{66.2}
\expandafter\def\csname res@size-27-2\endcsname{82.3}
\expandafter\def\csname res@size-27-3\endcsname{66.7}
\expandafter\def\csname res@size-4-2\endcsname{82.1}
\expandafter\def\csname res@size-4-3\endcsname{66.3}
\expandafter\def\csname res@size-9-2\endcsname{82.1}
\expandafter\def\csname res@size-9-3\endcsname{66.7}
\expandafter\def\csname res@text-best-2\endcsname{83.2}
\expandafter\def\csname res@text-best-3\endcsname{68.8}
\expandafter\def\csname res@text-best-model-2\endcsname{ModernBERT-large (fine-tuned)}
\expandafter\def\csname res@text-best-model-3\endcsname{ModernBERT-large (fine-tuned)}
\expandafter\def\csname res@toolkit-2\endcsname{94.9}
\expandafter\def\csname res@toolkit-3\endcsname{91.4}
\expandafter\def\csname res@toolkit-gap-2\endcsname{4.1}
\expandafter\def\csname res@toolkit-gap-3\endcsname{6.9}
\expandafter\def\csname res@train-utterances\endcsname{116{,}263}
\expandafter\def\csname res@vis-systems\endcsname{15}
\expandafter\def\csname res@vis-words\endcsname{89{,}935}
\expandafter\def\csname res@wordmaj-2\endcsname{80.7}
\expandafter\def\csname res@wordmaj-3\endcsname{62.0}
\makeatother

